Imaginary time evolution and ground state preparation using unitary multi-copy protocols

Efficient low-energy state preparation is a key objective in quantum computation and quantum simulation. Quantum imaginary-time evolution replaces real-time dynamics with imaginary-time dynamics, exponentially suppressing higher-energy eigenstates. We introduce deterministic unitary protocols that approximate imaginary-time evolution for ground state preparation. The protocols require multiple copies of the system, real-time evolution under the system Hamiltonian, and controlled-SWAP operations (or more general SWAP-generated unitaries). Our analysis focuses on two concrete circuit families: a tree architecture with provable polynomial-in-depth convergence but rapidly growing width, and a compact "hedge" architecture that achieves comparable accuracy with only polynomial width in a heuristic construction supported by numerics. Numerical evidence indicates that mid-circuit post-selection can accelerate convergence with practical success probabilities. Separately, we demonstrate that circuit volume can be traded for the shot complexity of post-circuit observable estimation in the ground state preparation setting. Finally, we outline concrete platform-specific implementations in which multi-copy registers and SWAP-mediated couplings are natural, illustrating how these hybrid analog-digital circuits can complement existing state-preparation methods in the near term.

==> tikzHedge.tex <==
% \begin{tikzpicture}[scale=0.65,
%   x=0.55cm, y=0.55cm,
%   wire/.style={very thick, line cap=round},
%   link/.style={very thick, line cap=round},
%   bdot/.style={circle, fill=blue!65, draw=none, minimum size=4.5pt, inner sep=0pt},
%   rdot/.style={circle, fill=red!80,  draw=none, minimum size=4.5pt, inner sep=0pt}
% ]

% % helper: vertical link with BLUE on top and RED on bottom
% \newcommand{\gate}[3]{%
%   \draw[link] (#1,-#2) -- (#1,-#3);
%   \node[bdot] at (#1,-#2) {};
%   \node[rdot] at (#1,-#3) {};
% }

% % 8 wires
% \def\xL{-0.5}
% \def\xR{15.5}
% \foreach \i in {0,...,7} {
%   \draw[wire] (\xL,-\i) -- (\xR,-\i);
% }

% % gates: (x, topwire, bottomwire), wires counted from 0 (top) to 7 (bottom)
% \gate{0}{0}{7}

% \gate{1}{1}{6}

% \gate{2}{0}{1}
% \gate{2}{6}{7}

% \gate{3}{1}{6}

% \gate{4}{2}{5}

% \gate{5}{1}{2}
% \gate{5}{5}{6}

% \gate{6}{0}{1}
% \gate{6}{2}{5}
% \gate{6}{6}{7}

% \gate{7}{1}{2}
% \gate{7}{5}{6}

% \gate{8}{2}{5}

% \gate{9}{3}{4}

% \gate{10}{2}{3}
% \gate{10}{4}{5}

% \gate{11}{1}{2}
% \gate{11}{3}{4}
% \gate{11}{5}{6}

% \gate{12}{0}{1}
% \gate{12}{2}{3}
% \gate{12}{4}{5}
% \gate{12}{6}{7}

% \gate{13}{1}{2}
% \gate{13}{3}{4}
% \gate{13}{5}{6}

% \gate{14}{2}{3}
% \gate{14}{4}{5}

% \gate{15}{3}{4}

% \end{tikzpicture}

\begin{tikzpicture}[scale=0.65,
  x=0.55cm, y=0.55cm,
  wire/.style={very thick, line cap=round},
  link/.style={very thick, line cap=round},
  bdot/.style={circle, fill=blue!65, draw=none, minimum size=4.5pt, inner sep=0pt},
  rdot/.style={circle, fill=red!80,  draw=none, minimum size=4.5pt, inner sep=0pt}
]

% helper: vertical link with BLUE on top and RED on bottom
\newcommand{\vlink}[3]{%
  \draw[link] (#1,-#2) -- (#1,-#3);
  \node[bdot] at (#1,-#2) {};
  \node[rdot] at (#1,-#3) {};
}

% 8 wires
\def\xL{-0.5}
\def\xR{15.5}
\foreach \i in {0,...,7} {
  \draw[wire] (\xL,-\i) -- (\xR,-\i);
}

% gates: (x, topwire, bottomwire)
\vlink{0}{0}{7}
\vlink{1}{1}{6}
\vlink{2}{0}{1}
\vlink{2}{6}{7}
\vlink{3}{1}{6}
\vlink{4}{2}{5}
\vlink{5}{1}{2}
\vlink{5}{5}{6}
\vlink{6}{0}{1}
\vlink{6}{2}{5}
\vlink{6}{6}{7}
\vlink{7}{1}{2}
\vlink{7}{5}{6}
\vlink{8}{2}{5}
\vlink{9}{3}{4}
\vlink{10}{2}{3}
\vlink{10}{4}{5}
\vlink{11}{1}{2}
\vlink{11}{3}{4}
\vlink{11}{5}{6}
\vlink{12}{0}{1}
\vlink{12}{2}{3}
\vlink{12}{4}{5}
\vlink{12}{6}{7}
\vlink{13}{1}{2}
\vlink{13}{3}{4}
\vlink{13}{5}{6}
\vlink{14}{2}{3}
\vlink{14}{4}{5}
\vlink{15}{3}{4}

\end{tikzpicture}

==> tikzTree.tex <==
\begin{tikzpicture}[scale = 0.65,
  x=1.35cm, y=0.55cm,
  wire/.style={very thick, line cap=round},
  link/.style={very thick, line cap=round},
  bdot/.style={circle, fill=blue!65, draw=none, minimum size=4.5pt, inner sep=0pt},
  rdot/.style={circle, fill=red!80,  draw=none, minimum size=4.5pt, inner sep=0pt}
]

% 8 wires
\def\xL{0}
\def\xR{3.2}
\foreach \i in {0,...,7} {
  \draw[wire] (\xL,-\i) -- (\xR,-\i);
}

% Column A: four adjacent links (1-2, 3-4, 5-6, 7-8)
\def\xa{0.5}
\foreach \top/\bot in {0/1, 2/3, 4/5, 6/7} {
  \draw[link] (\xa,-\top) -- (\xa,-\bot);
  \node[bdot] at (\xa,-\top) {};
  \node[rdot] at (\xa,-\bot) {};
}

% Column B: two links (1-3, 5-7)
\def\xb{1.5}
\foreach \top/\bot in {0/2, 4/6} {
  \draw[link] (\xb,-\top) -- (\xb,-\bot);
  \node[bdot] at (\xb,-\top) {};
  \node[rdot] at (\xb,-\bot) {};
}

% Column C: one link (1-5)
\def\xc{2.5}
\draw[link] (\xc,0) -- (\xc,-4);
\node[bdot] at (\xc,0) {};
\node[rdot] at (\xc,-4) {};

\end{tikzpicture}
